ATARS: An Aerial Traffic Atomic Activity Recognition and Temporal Segmentation Dataset

Traffic Atomic Activity which describes traffic patterns for topological intersection dynamics is a crucial topic for the advancement of intelligent driving systems. However, existing atomic activity datasets are collected from an egocentric view, which cannot support the scenarios where traffic activities in an entire intersection are required. Moreover, existing datasets only provide video-level atomic activity annotations, which require exhausting efforts to manually trim the videos for recognition and limit their applications to untrimmed videos. To bridge this gap, we introduce the Aerial Traffic Atomic Activity Recognition and Segmentation (ATARS) dataset, the first aerial dataset designed for multi-label atomic activity analysis. We offer atomic activity labels for each frame, which accurately record the intervals for traffic activities. Moreover, we propose a novel task, Multi-label Temporal Atomic Activity Recognition, enabling the study of accurate temporal localization for atomic activity and easing the burden of manual video trimming for recognition. We conduct extensive experiments to evaluate existing state-of-the-art models on both atomic activity recognition and temporal atomic activity segmentation. The results highlight the unique challenges of our ATARS dataset, such as recognizing extremely small objects' activities. We further provide comprehensive discussion analyzing these challenges and offer valuable insights for future direction to improve recognizing atomic activity in aerial view. Our source code and dataset are available at https://github.com/magecliff96/ATARS/

==> chapters/recycling.tex <==
\subsection{Dataset Comparison}
\begin{table*}[h!]
\centering
\scriptsize
\caption{Comparison with traffic datasets relevant to traffic pattern analysis for intersection traffic dynamics. For dataset focus, \textcolor{darkred}{Caption} represents captioning, \textcolor{darkorange}{OD} represents Object Detection, \textcolor{darkblue}{PR} represents Pattern Recognition, \textcolor{darkgreen}{TP} represents Trajectory Prediction, and \textcolor{darkteal}{TAS} represents Temporal Action Segmentation.
}\resizebox{0.98\linewidth}!{
\begin{tabular}
    {@{} c@{\;} | c@{\;} | c@{\;} | c@{\;} c@{\;} c@{\;} c@{\;} c@{\;} c@{\;} }
    \toprule
    \multirow{2}{*}{Dataset} &  
    \multirow{2}{*}{Perspective} &  
    \multirow{2}{*}{Dataset Focus} &  
    \multirow{2}{*}{Real Data} &  
    \multicolumn{1}{c}{Video Pattern} &  
    \multicolumn{1}{c}{Frame Pattern} &  
    \multirow{2}{*}{Trajectory} &  
    \multicolumn{1}{c}{Bounding} &  
    \multicolumn{1}{c}{Pedestrian}  
    \\  
    &  
    &  
    &  
    &  
    \multicolumn{1}{c}{Labels} &  
    \multicolumn{1}{c}{Labels} &  
    &  
    \multicolumn{1}{c}{Box} &  
    \multicolumn{1}{c}{Annotations}  
    \\  
    \hline
    Drama~\cite{malla2023drama} & \textcolor{darkblue}{First-person} & \textcolor{darkred}{Caption}, \textcolor{darkblue}{PR}, \textcolor{darkorange}{OD} & \cmark & \cmark & \xmark & \xmark & \cmark & \cmark  
    \\  
    HDD~\cite{ramanishka2018toward} & \textcolor{darkblue}{First-person} & \textcolor{darkblue}{PR}, \textcolor{darkorange}{OD} & \cmark & \cmark & \cmark & \xmark & \cmark & \xmark  
    \\  
    OATS~\cite{agarwal2023ordered} & \textcolor{darkblue}{First-person} & \textcolor{darkblue}{PR} & \cmark & \cmark & \xmark & \xmark & \xmark & \cmark  
    \\  
    TACO~\cite{kung2024action} & \textcolor{darkblue}{First-person} & \textcolor{darkblue}{PR} & \xmark & \cmark & \xmark & \xmark & \xmark & \cmark  
    \\  
    
    \hline
    UAVDT~\cite{du2018unmanned} & \textcolor{darkorange}{Drone} & \textcolor{darkorange}{OD} & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark  
    \\  
    VisDrone~\cite{} & \textcolor{darkorange}{Drone} & \textcolor{darkorange}{OD} & \cmark & \xmark & \xmark & \cmark & \cmark & \cmark  
    \\  
    
    \hline
    CitySim~\cite{zheng2024citysim} & \textcolor{darkgreen}{Top-down} & \textcolor{darkgreen}{TP} & \cmark & \xmark & \cmark & \cmark & \cmark & \xmark  
    \\  
    INTERACTION~\cite{zhan2019interaction} & \textcolor{darkgreen}{Top-down} & \textcolor{darkgreen}{TP} & \cmark & \xmark & \cmark & \cmark & \xmark & \cmark  
    \\  
    inD~\cite{bock2020ind} & \textcolor{darkgreen}{Top-down} & \textcolor{darkgreen}{TP} & \cmark & \xmark & \cmark & \cmark & \cmark & \cmark  
    \\  
    SinD~\cite{xu2022drone} & \textcolor{darkgreen}{Top-down} & \textcolor{darkgreen}{TP} & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark  
    \\  
    \hline
    CAROM~\cite{lu2023carom} & \textcolor{darkgreen}{Top-down} & \textcolor{darkgreen}{TP} & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark  
    \\  
    CAROM-OAA (ours) & \textcolor{darkgreen}{Top-down} & \textcolor{darkteal}{TAS}, \textcolor{darkblue}{PR}, \textcolor{darkgreen}{TP} & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark  
    \\  
    \bottomrule
\end{tabular}
}
%\vspace{8pt}
\label{table:dataset}
\vspace{-2mm}

\end{table*}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=1\linewidth]{img/topology2.png}
%     \caption{Example of multi-label atomic activity. The frame in (a) is labeled with v13+, v32, and p43, illustrating one vehicle is moving from z3 to z2, multiple vehicle from z1 to z3, and one pedesterian from c4 to c3. The frame in (b) is labeled with v31+. The label will change to v31 the moment the first vehicle exists the intersection.}
%     \label{fig:topology}
%      %\vspace{-5pt}
% \end{figure}

% Intro:
% Traffic pattern recognition and temporal action segmentation play a crucial role in understanding and modeling the behavior of vehicles and pedestrians in urban environments, with applications in 


% ability to capture the broader topology of intersections and constrains models' capacity to analyze topological traffic pattern dynamics. Without a comprehensive view of intersections, accurately recognizing the multi-label atomic activities of interacting agents in traffic scenes becomes challenging, 
% thereby reducing the effectiveness of downstream applications in traffic analysis and simulation.
% Top-down view () datasets provide a more comprehensive perspective of intersections but primarily focus on vehicle tracking, object recognition, or landscape segmentation, often lacking annotations for traffic pattern analysis.
% To address these limitations, many recent datasets~\cite{zhan2019interaction,bock2020ind,xu2022drone,zheng2024citysim} have explored Top-down view perspectives, which offer a more comprehensive view of traffic patterns at intersections. Top-down perspectives excel at capturing how vehicles and pedestrians interact in complex traffic scenarios at intersections. However, existing datasets that include Top-down view footage primarily focus on vehicle tracking~\cite{zhan2019interaction,zheng2024citysim}, object recognition~\cite{du2018unmanned,zhu2021detection}, or landscape segmentation~\cite{xia2018dota}. 

% These datasets often lack the pattern annotations necessary for high-level analysis of traffic dynamics. Moreover, while Top-down view datasets offer an improved perspective over ego-centric views, vehicles and pedestrians appear significantly smaller in aerial footage, making action segmentation more challenging. The absence of structured annotations further limits progress in topological traffic pattern recognition and temporal action segmentation, restricting models' ability to accurately classify and analyze interaction behaviors.

% CAROM-MAA is introduced as a Top-down view view dataset that offers frame-wise annotations for both vehicle and pedestrian activities, addressing the limitations of ego-centric MAA datasets and emphasizing small object recognition.
% To bridge this gap, we introduce CAROM-MAA, a Top-down view dataset designed to facilitate research in traffic pattern recognition and temporal action segmentation. 
% Figure~\ref{fig:teaser} illustrates the tasks and unique challenges CAROM-MAA addresses. 
% Unlike existing MAA datasets, which are constrained by their video-level label granularity, CAROM-MAA provides frame-wise granularity, containing both vehicle and pedestrian activity labels for temporal action segmentation tasks. 
% Captured from a drone perspective, the dataset is designed to study the entire intersection, encompassing multiple small agents in the scene. However, the small size of these agents presents a challenge often overlooked in conventional datasets, where agents appear larger and are more easily detectable. 
% By structuring the dataset to emphasize small object recognition in action segmentation, CAROM-MAA enables a more detailed analysis of intersection behaviors, which is crucial for advancing traffic flow simulation and anomaly detection. 

% Related work:

% % Various methods for video-level traffic pattern recognition have been proposed, including slot-attention models like Action-Slot for atomic activities, SlowFast networks for improved temporal modeling, and graph-based approaches like ORN and ARG for group activity recognition.
% To capture traffic patterns in intersections,many methods for video-level traffic pattern recognition were proposed. Slot-attention based methods such as Action-Slot~\cite{kung2024action} utilizes slot attention mechanisms to capture atomic activities describing complex urban interactions. To improve temporal modeling for complex situations, several methods, such as SlowFast~\cite{feichtenhofer2019slowfast}, Networks was proposed. Lastly, ORN~\cite{baradel2018object} introduce graph-based reasoning for group activity recognition, which inspired methods such as ARG~\cite{wu2019learning}.

% % Beyond video-level traffic pattern recognition, temporal action segmentation models like MS-TCN and MS-TCN++ enable structured activity analysis, while transformer-based methods like ASFormer, PointTAD, and MLAD improve long-term dependency modeling and multi-label action recognition.
% In addition to traffic pattern recognition methods that analyze data at video-level, temporal action segmentation models also played an important role in structured activity analysis. MS-TCN~\cite{farha2019ms} and MS-TCN++~\cite{li2020ms} pioneer multi-stage temporal convolutional networks for action segmentation, making them effective at recognizing structured traffic activities. With the advent of transformer, ASFormer~\cite{yi2021asformer} applies transformers to frame-level segmentation to model long-term dependencies in traffic movement. PointTAD~\cite{tan2022pointtad} proposes learnable query points for multi-label temporal action detection, allowing for flexible recognition of overlapping road user actions. To model multi-label action dependencies, MLAD~\cite{tirupattur2021modeling} was proposed.

% % CAROM-MAA enhances traffic pattern recognition by integrating multi-label atomic action annotations with frame-level granularity from a top-down perspective, providing unique challenges for evaluating state-of-the-art recognition and segmentation models.
% By incorporating multi-label atomic action annotations from a top-down perspective with frame-level granularity, CAROM-MAA offers rich data for traffic pattern recognition at the frame level. Unlike datasets that primarily focus on trajectories or coarse action patterns, our topology-aware activity annotations, combined with a top-down perspective video data, present unique challenges that offer deeper insights into the performance of state-of-the-art traffic pattern recognition and temporal segmentation models for traffic pattern recognition.

%\textcolor{red}{list what we have done for the dataset and the advantage of our data here, not the annotation. }
% ability to capture the broader topology of intersections and constrains models' capacity to analyze topological traffic pattern dynamics. Without a comprehensive view of intersections, accurately recognizing the multi-label atomic activities of interacting agents in traffic scenes becomes challenging, 

% To address these limitations, many recent datasets~\cite{zhan2019interaction,bock2020ind,xu2022drone,zheng2024citysim} have explored Top-down view perspectives, which offer a more comprehensive view of traffic patterns at intersections. Top-down perspectives excel at capturing how vehicles and pedestrians interact in complex traffic scenarios at intersections. However, existing datasets that include Top-down view footage primarily focus on vehicle tracking~\cite{zhan2019interaction,zheng2024citysim}, object recognition~\cite{du2018unmanned,zhu2021detection}, or landscape segmentation~\cite{xia2018dota}. 



%Our methodology also supports multi-label ordered atomic activity recognition. Unlike traditional annotation techniques that focus on trajectories or bounding boxes, our approach explicitly encodes the spatial origin-destination relationship and the nature of the road user. This allows for simultaneous recognition and classification of multiple fine-grained traffic activities while maintaining a strong contextual foundation for advanced traffic scene analysis. Furthermore, CAROM-MAA leverages the multi-label atomic activity (MAA) labeling system, which provides an additional advantage over datasets such as SinD. While both approaches offer video- and frame-level pattern labels, MAA explicitly models temporal dependencies and interactive relationships, enabling a structured decomposition of scenarios into ordered atomic activities. This allows for the representation of complex interactions, such as yielding or priority-based actions, which are not explicitly captured in SinD. By grounding each activity in the underlying road topology and actor roles, CAROM-MAA enables efficient scenario retrieval, yielding a more scalable and interpretable annotation framework. Additionally, CAROM-MAA distinguishes itself by providing comprehensive annotation, including real data, both video- and frame-level pattern labels, trajectory data, bounding boxes, and pedestrian tracking. By incorporating MAA labeling, CAROM-MAA further enhances motion prediction, behavior modeling, and intersection safety analysis, making it a robust framework for fine-grained traffic scenario understanding.



%Table~\ref{table:dataset} compares our dataset, CAROM-MAA, with existing datasets. Most datasets provide either bounding boxes or trajectory annotations but lack video- or frame-level Road Topology Pattern labels. While egocentric datasets such as Drama~\cite{malla2023drama} and HDD~\cite{ramanishka2018toward} contains various descriptive video pattern labels or captions, their annotations are of video-level granularity and lack topologically aware annotations and detailed trajectory tracking. Meanwhile, while drone-view datasets such as UAVDT~\cite{du2018unmanned} and VisDrone~\cite{zhu2018vision} contain bounding boxes and pedestrian tracking, they lack traffic pattern labels. While some top-down view datasets such as INTERACTION~\cite{zhan2019interaction} and SinD~\cite{xu2022drone} do contain traffic pattern labels in addition to bounding boxes and trajectory annotations, these labels are neither descriptive nor topological aware. Our CAROM-MAA is the only dataset to contains both video- and frame-level road topology pattern labels, while inheriting trajectory data and bounding boxes from CAROM. By incorporating MAA labeling, CAROM-MAA further distinguishes itself from datasets such as SinD or Road by explicitly annotating topology aware interactive behaviors. This allows for more refined traffic behavior modeling and analysis, making CAROM-MAA a valuable dataset for fine-grained traffic scenario understanding.


% method

    % \item \textbf{Data Structure and Review:} Each annotated instance is documented on a spreadsheet, with each row representing individual segment instance and columns recording start and end frames of each patterns. Two columns are assigned to every class, representing their corresponding start and end frame. A rigorous review process was conducted to verify that the conssistent and accurate annotations.

    % Unlike previous works, our annotation process is focused on the status of the intersection. Annotation begins when a vehicle or pedestrian enters the intersection, which is defined as the area bounded by the outer line of the pedestrian crossings, or by the edges of the four corners if sidewalk crossings are not present. An example of this definition is outlined in Figure~\ref{fig:teaser} (a). Unlike previous work, which is ego-vehicle oriented, our annotation is intersection-oriented. Each frame is examined to determine whether an AA definition is met, such as a pedestrian moving from corner c1 to corner c2. For example, in Figure~\ref{fig:teaser} (a), frames showing a group of vehicles moving from z1 to z3 are annotated as 13v+, where `+' indicates the presence of multiple vehicles. However, once all but one vehicle have exited the intersection, the annotation changes to 13v.
% The start frame of a vehicle's AA is defined as the frame when the front of the vehicle passes the outer line on the crossing, or when the vehicle resumes motion after coming to a stop. The end frame is marked as the moment when the vehicle's rear crosses the outer white line of the pedestrian crossing. In cases where a turning vehicle moves forward into the intersection, stops, and then initiates their turning maneuver into their destination roadway, the previous forward motion is not annotated. Instead, the start frame is adjusted to when the turning action begins, as only moving forward is not an indicator of a turning pattern. These stopped durations are also not annotated as positive (as no motion is occurring). For pedestrians, the start frame is recorded when they exit a corner and enter the intersection, while the end frame is marked when they leave the crossing by reaching the opposite corner.
    
    % \item \textbf{Group Annotations :} \hank{shorten this by stating "we follow xxx. Specifically, xxx."}The annotation differentiates between singular and group activities. A singular action (e.g., 12v or 21p) is recorded when one traffic participant is involved in that moving pattern. If multiple traffic participants execute the same action concurrently, it is annotated as a group label (e.g., 12v+) while it involves multiple participants. The group segment transitions to a new singular action (e.g., 12v) in a frame where all but one participant of this pattern remains in the intersection area, regardless of the starting condition. The start and end annotations of these transitions between singular and group annotations do not overlap to ensure clarity and consistency.
